The MOSDEF-LRIS Survey: Detection of Inflowing Gas Towards Three Star-forming Galaxies at z ~ 2

We report on the discovery of cool gas inflows towards three star-forming galaxies at $\left<z\right>\sim$ 2.30. Analysis of Keck Low-Resolution Imaging Spectrometer spectroscopy reveals redshifted low-ionisation interstellar (LIS) metal absorption lines with centroid velocities of 60 - 130 km $\rm{s}^{-1}$. These inflows represent some of the most robust detections of inflowing gas into isolated, star-forming galaxies at high redshift. Our analysis suggests that the inflows are due to recycling metal-enriched gas from previous ejections. Comparisons between the galaxies with inflows and a larger parent sample of 131 objects indicate that galaxies with detected inflows may have higher specific star-formation rates (sSFR) and star-formation-rate surface densities. However, when additional galaxies without robustly detected inflows based on centroid velocity but whose LIS absorption line profiles indicate large red-wing velocities are considered, galaxies with inflows do not show unique properties relative to those lacking inflows. Additionally, we calculate the covering fraction of cool inflowing gas as a function of red-wing inflow velocity, finding an enhancement in high sSFR binned galaxies, likely due to an increase in the amount of recycling gas. Together, these results suggest that the low detection rate of galaxies with cool inflows is primarily related to the viewing angle rather than the physical properties of the galaxies.

==> arxiv inflow/Spectral_Windows.tex <==
\begin{table}
  \centering
  \caption{Spectral Windows}
  \label{tbl:spectral_windows}
  \begin{threeparttable}
    \begin{tabular}{lccc}
        \hline
        \hline
        Line  & $\lambda_{\rm{rest}}$ (\AA)\tnote{a} & Blue Window (\AA)\tnote{b} & Red Window (\AA)\tnote{b}\\
        \hline
   
        Ly$\alpha$   & 1215.67 & 1195 - 1202 & 1225 - 1235\\
        \ion{Si}{II} & 1260.42 & 1245 - 1252 & 1270 - 1275\\
        \ion{O}{II} + \ion{Si}{II} & 1303.27 & 1285 - 1293 & 1312 - 1318\\
        \ion{C}{II}  & 1334.53 & 1320 - 1330 & 1342 - 1351\\
        \ion{Si}{II} & 1526.71 & 1512 - 1520 & 1535 - 1540\\
    \hline
    \end{tabular}
    \begin{tablenotes}
        \item[a] Rest-frame vacuum wavelength, taken from the Atomic Spectra Database website of the National Institute of Standards and Technology (NIST), https://www.nist.gov/pml/atomic-spectra-database.
        \item[b] Wavelength window over which continuum fitting was performed.
    \end{tablenotes}

  \end{threeparttable}
\end{table}

==> arxiv inflow/Vhalo.tex <==
\begin{table*}
  \centering
  \caption{Inflow Velocities}
  \label{tbl:halo_vel}
  \begin{threeparttable}
    \begin{tabular}{llccccc}
        \hline
        \hline
        Field & V4ID & log($M_{\rm{halo}}/M_{\odot}$) & log$(M_{\star}/M_{\odot})$ & $v_{\rm{cen, red}}$\tnote{a} & $v_{\rm{max, red}}$\tnote{b} & $V_{\rm{stream}}$\tnote{c}\\
        & & & & [km s$^{-1}$] & [km s$^{-1}$] & [km s$^{-1}$]\\
        \hline
        COSMOS  & 4156  & 11.53$\pm$0.07 &  9.11$\pm$0.04 & 250$\pm$100 & 413$\pm$51 &  98$\pm$11\\
        GOODS-S & 40218 & 11.90$\pm$0.09 &  9.79$\pm$0.04 & 400$\pm$80  & 720$\pm$36 & 145$\pm$13\\
        GOODS-S & 40768 & 12.06$\pm$0.06 & 10.09$\pm$0.01 & 450$\pm$87  & 766$\pm$61 & 158$\pm$11\\
        \hline

    \end{tabular}
    \begin{tablenotes}
        \item[a] Centroid velocity of the inflowing gas (See Section \ref{sec:decomp}).
        \item[b] Maximum inflow velocity (See Section \ref{sec:vels}).
        \item[c] Cold stream inflow velocity
    \end{tablenotes}

  \end{threeparttable}
\end{table*}
